Exploiting Data Sparsity in Secure Cross-Platform Social Recommendation

Social recommendation has shown promising improvements over traditional systems since it leverages social correlation data as an additional input. Most existing work assumes that all data are available to the recommendation platform. However, in practice, user-item interaction data (e.g.,rating) and user-user social data are usually generated by different platforms, and both of which contain sensitive information. Therefore, "How to perform secure and efficient social recommendation across different platforms, where the data are highly-sparse in nature" remains an important challenge. In this work, we bring secure computation techniques into social recommendation, and propose S3Rec, a sparsity-aware secure cross-platform social recommendation framework. As a result, our model can not only improve the recommendation performance of the rating platform by incorporating the sparse social data on the social platform, but also protect data privacy of both platforms. Moreover, to further improve model training efficiency, we propose two secure sparse matrix multiplication protocols based on homomorphic encryption and private information retrieval. Our experiments on two benchmark datasets demonstrate the effectiveness of S3Rec.

==> protocols/PIR.tex <==
% \protocol{$\vec{q}\gets \mathsf{PIR.Query}(i)$}{
% s_j =(s_{j,i})_{i\in[m]}\\
% l\gets \lceil d\cdot m/ 2^c \rceil\\
% \text{Parse~}(s_1,...,s_d)\text{~as~}(s^\prime_1,...,s^\prime_d)\text{~vectors~in~}\bin^m\\
% \forall j\in[l], m_j \gets \sum_{i\in [2^c]}2^{-c}\cdot s_j[i]\cdot x^i\in R_t\\
% \forall j\in[l], q_j\gets \mathsf{Enc}_{sk}(m_j)\\
% \vec{q}=(q_j)_{j\in[l]}\in R_q^l
% }


\fbox{
  \begin{minipage}{0.95\linewidth}
    

    \smallskip
    \underline{Parameters}: $d\in[1,\log n], m = n^{1/d}$, compression $c\in[0, \log_2 N]$.
    
    \medskip
    \underline{$\mathsf{PIR.Query}(i)$}
    
    \smallskip
    \procedure[linenumbering, width=\linewidth, codesize=\normalsize]{}{
    \textrm{Generate~}s_j =(s_{j,i})_{i\in[m]}, \textrm{the~} d \textrm{-th selections vector in~} \bin^m\\
    l\gets \ceil{d\cdot m/ 2^c}\\
    \textrm{Parse~}(s_1,...,s_d)\textrm{~as~}(s^\prime_1,...,s^\prime_d)\textrm{~vectors in~}\bin^{2^c}\\
    \forall j\in[l], m_j \gets \sum_{i\in 2^c}(2^{-c}\mod t)\cdot s_j[i]\cdot x^i\in R_t\\
    \forall j\in[l], q_j\gets \mathsf{Enc}_{sk}(m_j)\\
    \vec{q}=(q_j)_{j\in[l]}\in R_q^l\\
    \pcreturn \vec{q}
    }
    
    \medskip
    \underline{$\mathsf{PIR.Expand}(q)$}
    
    \smallskip
    \procedure[linenumbering, width=\linewidth, codesize=\normalsize]{}{
    l\gets \ceil{d\cdot m/2^c}\\
    \mathsf{ciphertexts}\gets []\\
    \pcfor j \in \set{1,\ldots,l}, \mathsf{ctxts}=[q_j=(c_0, c_1)] \pcdo \\
    \t\pcfor a \in \set{0,\ldots,c-1} \pcdo \\
    \t\t \pcfor b \in \set{0,\ldots,2^a-1} \pcdo\\
    \t\t\t\textrm{Let~} c_k^\prime \gets c_0 + \mathsf{Sub}_{2^{c-a}+1}(c_0)\\
    \t\t\t\textrm{Let~} c_{k+2^a}^\prime \gets c_1 +\mathsf{Sub}_{2^{c-a}+1}(c_1)\\
    \t\t\pcendfor\\
    \t\t \mathsf{ctxts}=[c_0^\prime, ..., c_{2^{a+1}-1}^\prime]\\
    \t\pcendfor\\
    \t\mathsf{ciphertexts}\gets\mathsf{ciphertexts} \| \mathsf{ctxts}\\
    \pcendfor\\
    \textrm{Let~}\vec{s}\gets\mathsf{ciphertexts}\\
    \pcreturn \vec{s}
    }
    
    
    \medskip
    \underline{$\mathsf{PIR.Response}(\mathsf{DB}, \vec{s})$}
    
    \smallskip
    \procedure[linenumbering, width=\linewidth, codesize=\normalsize]{}{
    \forall s_i\in\vec{s}, \textrm{let~}\mathsf{DB}_i =\bigoplus_{j=0}^m\mathsf{DB.Get}(i,j)\otimes s_i[j]\\
    \pcreturn r:=\mathsf{DB}_i
    }
    
    \medskip
    \underline{$\mathsf{PIR.Extract}(r)$}
    
    \smallskip
    \procedure[linenumbering, width=\linewidth, codesize=\normalsize]{}{
    \forall i\in\set{1,\ldots, d}, \textrm{let~}r:=\mathsf{Dec}_{sk}(r) \bmod 2^l\\
    \pcreturn \mathsf{DB}_i:=r
    }
    
    % \smallskip\textbf{Algorithm $\vec{q}\gets \mathsf{PIR.Query}(i)$}:
    % \begin{enumerate}
    %     \item Generate $s_j =(s_{j,i})_{i\in[m]}$ the $d$ selections vector in $\{0,1\}^m$.
    %     \item $l\gets \lceil d\cdot m/ 2^c \rceil$
    %     \item Parse $(s_1,...,s_d)$ as $(s^\prime_1,...,s^\prime_d)$ vectors in $\{0,1\}^{2^c}$.
    %     \item $\forall j\in[l], m_j \gets \sum_{i\in 2^c}(2^{-c}\mod t)\cdot s_j[i]\cdot x^i\in R_t$.
    %     \item $\forall j\in[l], q_j\gets \mathsf{Enc}_{sk}(m_j)$.
    %     \item $\vec{q}=(q_j)_{j\in[l]}\in R_q^l$.
    % \end{enumerate}
    
    % \smallskip\textbf{Algorithm $\vec{s}\gets \mathsf{PIR.Expand}(q)$}:
    % \begin{enumerate}
    %     \item $l\gets \lceil d\cdot m/2^c\rceil$.
    %     \item $\mathsf{ciphertexts}\gets []$.
    %     \item For $j=1$ to $l$, $\mathsf{ctxts}=[q_j=(c_0, c_1)]$,
    %     \begin{enumerate}
    %         \item For $a=0$ to $c-1$,
    %         \begin{enumerate}
    %             \item For $b=0$ to $2^a-1$, $c_0\gets\mathsf{ctxts}[b]$, $c_1\gets x^{-2^a}\cdot c_0$, $c_k^\prime \gets c_0 + \mathsf{Sub}_{2^{c-a}+1}(c_0)$, $c_{k+2^a}^\prime \gets c_1 + \mathsf{Sub}_{2^{c-a}+1}(c_1)$.
    %             \item $\mathsf{ctxts}=[c_0^\prime, ..., c_{2^{a+1}-1}^\prime]$
    %         \end{enumerate}
    %         \item $\mathsf{ciphertexts}\gets\mathsf{ciphertexts} \| \mathsf{ctxts}$
    %     \end{enumerate}
    %     \item Let $\vec{s}=\mathsf{ciphertexts}$.
    % \end{enumerate}
    
    % \smallskip\textbf{Algorithm $r\gets \mathsf{PIR.Response}(\mathsf{DB}, \vec{s})$}:
    % \begin{enumerate}
    %     \item For $s_i\in\vec{s}$, let $\mathsf{DB}_i =\bigoplus_{j=0}^m\mathsf{DB.Get}(i,j)\otimes s_i[j]$. At the end, there's only one value left in $\mathsf{DB}$.
    %     % \mathsf{Enc}_{sk}(s_i)\cdot\mathsf{DB}_i)
    %     \item Let $r:=\mathsf{DB}$.
    % \end{enumerate}
    
    % \smallskip\textbf{Algorithm $\mathsf{DB}_i\gets \mathsf{PIR.Extract}(r)$}:
    % \begin{enumerate}
    %     \item For $i\in[1, d]$, $r:=\mathsf{Dec}_{sk}(r) \mod 2^l$.
    %     \item Let $\mathsf{DB}_i:=r$.
    % \end{enumerate}
    
  \end{minipage}
}

==> protocols/dense_m_diagonal_m.tex <==
% \fbox{
%   \begin{minipage}{0.95\linewidth}
%     $\llbracket \textbf{Z}\rrbracket \gets\mathsf{MatrixMul}(\textbf{X}, \textbf{Y})$, where $\textbf{X}\in\mathbb{R}^{k\times m}, \textbf{Y}\in\mathbb{R}^{m\times m}$, and $\textbf{Y}$'s location vector $l_y$ is public.
    
%     \smallskip\textbf{Offline Phase:}
%     \begin{itemize}
%         \item Generates $k|l_y|$ Beaver's triples for $\mathsf{Mul}$ instances.
%     \end{itemize}
%         \textbf{Online Phase:}
%     \begin{itemize}
%         \item For all locations $(i,j)\in l_y$, $P_1$ pushes $y_{i,j}$ into $T_y(j)$.
%         \item \pcfor $0\leq i< k$, \pcdo
%         \begin{itemize}
%             \item[$\circ$] $P_1$ lets $T_y=\emptyset$.
%             \item[$\circ$] For all $0\leq a < m$ and $0\leq b < m$, if $(i,a)\in l_y$, $P_0$ pushes $x_{a,b}$ into $T_x(a)$.
%             \item[$\circ$] For all all $0\leq j< m$, first let $\llbracket z_{i,j}\rrbracket =0$,
%             \begin{itemize}
%                 \item Then for all values $v\in T_x(i)$ and $u\in T_y(j)$, $P_0$ invokes $\llbracket v\rrbracket \gets\mathsf{Shr}(v)$, and $P_1$ invokes $\llbracket u\rrbracket \gets\mathsf{Shr}(u)$. Afterwards, both $P_0$ and $P_1$ invoke $\llbracket z_{i,j}\rrbracket =\mathsf{Add}(\mathsf{Mul}(\llbracket v\rrbracket ,\llbracket u\rrbracket ), \llbracket z_{i,j}\rrbracket )$.
%             \end{itemize}
%         \end{itemize}
%         \item Return $\llbracket \textbf{Z}\rrbracket $.
%     \end{itemize}
%   \end{minipage}
% }
 
\begin{pcvstack}[center, boxed]

\procedure[linenumbering]{\textbf{Protocol}: $\llbracket \textbf{Z}\rrbracket \gets\mathsf{MatrixMul}(\textbf{X}, \textbf{Y})$}{
P_0, P_1\text{~jointly generate~} km^2 \text{~Beaver's triples}\pclb
\pcintertext[dotted]{Offline Completed}
\forall (i,j)\in l_y, P_1 \text{~pushes~} y_{i,j} \text{~into~} T_y(j)\\
\pcfor j\in[k] \pcdo\\
\t P_1 \text{~lets~} T_y=\emptyset\\
\t \forall a\in[m], b\in[m], \text{if~}(i,a)\in l_y, P_0 \text{~pushes~} x_{a,b} \text{~into~} T_x(a)\\
\t \pcfor j\in[m] \pcdo\\
\t\t \text{Both parties let~} \llbracket z_{i,j}\rrbracket=0, \text{then, for all values } v\in T_x(i), u\in T_y(j)\\
\t\t P_0\text{~invokes~} \llbracket v\rrbracket\gets\mathsf{Shr}(v), P_1\text{~invokes~} \llbracket v\rrbracket\gets\mathsf{Shr}(u)\\
\t\t \llbracket z_{i,j}\rrbracket =\mathsf{Add}(\mathsf{Mul}(\llbracket v\rrbracket,\llbracket u\rrbracket ), \llbracket z_{i,j}\rrbracket)\\
\t \pcendfor\\
\pcendfor
}

\end{pcvstack}

==> protocols/dense_m_sparse_m.tex <==
% \fbox{
%   \begin{minipage}{0.95\linewidth}
%     $\llbracket \textbf{Z}\rrbracket \gets\mathsf{MatrixMul}(\textbf{X}, \textbf{Y})$, where $\textbf{X}\in\mathbb{R}^{k\times m}$, $\textbf{Y}\in\mathbb{R}^{m\times m}$.

%     \smallskip\textbf{Offline Phase}:
%     \begin{enumerate}
%         \item $P_0$ generates an additive HE key pair $(pk, sk)$, then sends $pk$ to $P_1$.
%     \end{enumerate}
    
%     \smallskip\textbf{Online Phase}:
%     \begin{enumerate}
%         \item For all $0\leq i< k$ and $0\leq j< m$, $P_0$ lets $e_{i,j}=\mathsf{Enc}(pk,x_{i,j})$, and $\textbf{E}$ be the encrypted matrix.
%         \item For all $(i,j)\in l_y$, $P_1$ pushes $y_{i,j}$ into $T_y(j)$.
%         \item For all $(i,j)\in l_y$, $P_1$ invokes $q_{i,j}\gets\mathsf{PIR.Query}(i+jk)$. Afterwards, $P_1$ sends the query set (denote as $\textbf{q}$) to $P_0$.
%         \item For all $q_{i,j}\in \textbf{q}$, $P_0$ generates the reply $r_{i,j}\gets\mathsf{PIR.Response}(\textbf{E}, q_{i,j})$. Afterwards, $P_0$ returns the reply set (denote as $\textbf{r}$) to $P_1$.
%         \item For all $r_{i,j}\in \textbf{r}$, $P_1$ invokes $e_{i,j}\gets\mathsf{PIR.Extract}(r_{i,j})$ and pushes $e_{i,j}$ into $T^\prime_e(i)$.
%         \item For all $0\leq i< k$ and $0\leq j< m$,
%         \begin{enumerate}
%             \item $P_0$ initialises $\beta_{i,j}=\mathsf{Enc}_{pk}(0)$.
%             \item For all values $v\in T^\prime_e(i)$ and $u\in T_y(j)$, $P_0$ invokes $\beta_{i,j}=v\otimes u \oplus \beta_{i,j}$.
%             \item $P_0$ generates a random number $g_{i,j}\in\mathbb{Z}_\delta$, and lets $\beta_{i,j}=g_{i,j}\oplus \beta_{i,j}$.
%             \item $P_0$ sends $\beta_{i,j}$ to $P_1$, and lets $\llbracket z_{i,j}\rrbracket _0=-g_{i,j}$.
%         \end{enumerate}
%         \item $P_1$ decrypts all receiving messages and lets $\llbracket z_{i,j}\rrbracket _1=\mathsf{Dec}_{sk}(\beta_{i.j})$.
%         \item Return $\llbracket \textbf{Z}\rrbracket $.
%     \end{enumerate}
%   \end{minipage}
% }

\begin{pcvstack}[center, boxed]

\procedure[linenumbering]{\textbf{Protocol}: $\llbracket \textbf{Z}\rrbracket \gets\mathsf{MatrixMul}(\textbf{X}, \textbf{Y})$}{
P_0\text{~generates an additive HE key pair~} (\pk,\sk) \text{~, then sends~}\pk \text{~to~} P_1\pclb
\pcintertext[dotted]{Offline Completed}
% 
\forall i\in[k], j\in[m], P_0 \text{~lets~} e_{i,j}=\enc(\pk,x_{i,j}), \text{~and lets~} \textbf{E} \text{~be the encrypted matrix}\\
\forall (i,j)\in l_y, P_1 \text{~pushes~} y_{i,j} \text{~into~} T_y(j),
\text{also}, P_1 \text{~invokes~} q_{i,j}\gets\mathsf{PIR.Query}(i+jk)\\
% 
P_1 \text{~sends the query set (denoted as~}\textbf{q}\text{) to~} P_0\\
\forall q_{i,j}\in\textbf{q}, P_0\text{~invokes~} r_{i,j}\gets\mathsf{PIR}.\mathsf{Response}(\textbf{E}, q_{i,j}).\\
P_0 \text{~sends the response set (denoted as~}\textbf{r}\text{) to~} P_1\\
\forall r_{i,j}\in\textbf{r}, P_1\text{~invokes~} e_{i,j}\gets\mathsf{PIR}.\mathsf{Extract}(r_{i,j}) \text{~and~pushes~} e_{i,j} \text{~to~} T^\prime_e(i)\\
\pcfor i\in[k], j\in[m] \pcdo\\
\t P_0 \text{~lets~} \beta_{i,j}=\enc_\pk(0)\\
\t \forall v\in T^\prime_e(i), u\in T_y(j), P_0\text{~invokes~}\beta_{i,j} =v\otimes u\oplus \beta_{i,j}\\
\t P_0\text{~samples random numbers~} g_{i,j}\sample\mathbb{Z}_\delta, \text{then lets} \beta_{i,j}=g_{i,j}\oplus\beta_{i,j}\\
\t P_0 \text{~sends~} \beta_{i,j} \text{~to~} P_1, \text{then lets} \llbracket z_{i,j}\rrbracket_0= -g_{i,j}\\
\pcendfor\\
P_0 \text{decrypts all receving messages and lets~} \llbracket z_{i,j}\rrbracket_1=\dec_\sk(\beta_{i,j})\\
\pcreturn \llbracket Z\rrbracket
}

\end{pcvstack}

==> protocols/social_term_protocol.tex <==
\protocol{$\mathsf{ST}-\mathsf{MPC}(\gamma, \textbf{U}, \textbf{D}, \textbf{E}, \textbf{S})$}{%
\llbracket\textbf{R}^{(0)}\rrbracket\gets\mathsf{MatrixMul}(\gamma\textbf{U}/2, \textbf{D}^T+ \textbf{E}^T)\\
\llbracket\textbf{R}^{(1)}\rrbracket\gets\mathsf{MatrixMul}(-\gamma\textbf{U}, \textbf{S}^T)\\        \llbracket\textbf{R}\rrbracket\gets\mathsf{Add}(\llbracket\mathbf{R}^{(0)}\rrbracket,\llbracket\mathbf{R}^{(1)}\rrbracket)\\
\pcreturn \mathsf{Rec}(\llbracket\textbf{R}\rrbracket)\text{~to~}P_0
}

==> sections/a-1.tex <==
\section{Private Information Retrieval (PIR)}

Our protocol requires a bandwidth-efficient single-server PIR scheme. Specifically, in our work, we use the famous Seal PIR  \cite{Angel2018PIRWC}, which additionally leverages levelled homomorphic encryption scheme Fan-Vercauteren (FV) \cite{Fan2012SomewhatPF}. Slightly different from the standard PIR scheme, Seal-PIR further allows the client to send a compressed query to the server, which is then decompressed on the server by $\mathsf{PIR.Expand}$ algorithm. In general, Seal-PIR consists of four algorithms (see Figure \ref{fig:PIR}):
\begin{equation*}
    (\mathsf{PIR.Query}, \mathsf{PIR.Expand}, \mathsf{PIR.Response}, \mathsf{PIR.Extract}).
\end{equation*}


\begin{figure}[ht]
  \input{protocols/PIR}
  \caption{Seal-PIR algorithms, where we denote the number of entries in the database as $n$, and a user-defined recursion level as $d$. Also we use $\otimes$ to denote the homomorphic operation of plaintext-ciphertext multiplication $\oplus$ to denote the homomorphic operation of ciphertext addition. We also use $\mathsf{DB.Get}(i, j)$ to indicate get the $i$th dimension vector's $j$th value. }
  \label{fig:PIR}
\end{figure}

In particular, we consider single-server PIR with a computationally bounded adversary.
% 
The security definition is given below,
% 
\begin{definition}[Security of Computational PIR]
    Let $\mathcal{F}_\mathsf{PIR}$ be the query function which takes input as an index in $[|\mathsf{DB}|]$, where $\mathsf{DB}$ is the target database, and let $r$ be the user's random coins.
    % 
    Then for every distinct indices $i, j \in[|\mathsf{DB}|]$, and for every probabilistic polynomial-time adversary $\mathcal{A}$ bounded by security parameter $\lambda$, 
    % 
    \begin{equation*}
        |\Pr_r[\mathcal{A}(1^\lambda, \mathcal{F}_\mathsf{PIR}(i, r))=1]-\Pr_r[\mathcal{A}(1^\lambda, \mathcal{F}_\mathsf{PIR}(j, r))=1]|\leq\mathsf{negl}(\lambda).
    \end{equation*}
\end{definition}

Since the construction of Seal-PIR replies on FV, now we show the details of the FV scheme.

\smallskip\noindent\textbf{Fan-Vercauteren (FV)}. FV is a levelled homomorphic encryption scheme, where plaintexts are represented as polynomials of degree at most $N$, and integer coefficients modulo $t$. More specifically, the plaintext polynomials are from the quotient ring $R_t = \mathbb{Z}_t[x]/(x^N + 1)$, where $N$ is a power of 2, and $t$ is the plaintext modulus that determines how many data can a single FV plaintext represents. The ciphertexts in FV comprises of two polynomials from ring $R_q = \mathbb{Z}_q[x]/(x^N + 1)$, where $q$ is the coefficient modulus affecting the noise budget of a ciphertext and the security level of the entire cryptosystem. As operations such as addition or multiplication are performed, the noise of the output ciphertext grows based on the noise of the operands and the operation being performed. For the purpose of PIR, we care about the following operations:
\begin{equation*}
    p(x^k)=\mathsf{Sub}_k(c),
\end{equation*}
where $c$ is a ciphertext encrypting a polynomial $p(x)$,  and $k$ is an odd integer. For instance, if $c$ encrypts the polynomial $p(x)=x^3 + 4x$,  $\mathsf{Sub}_2(c)$ returns $(x^2)^3+4x^2 = x^6+4x^2$.



==> sections/a-2.tex <==
\section{Security Proofs}

First, we give the formal definitions of computational indistinguishability, simulation-based security (which is a popular tool for proving secure computation security), and IND-CPA security (indistinguishable chosen-plaintext attack). Then we use these definitions to prove lemma 1 and lemma 2.

\subsection{Definitions and Tools}


\begin{definition}[Computational Indistinguishability]
Let $a\in\{0,1\}^*$ be the inputs from participants, and $\lambda\in\mathbb{N}$ be the security parameter, two probability functions 
	$\{\mathcal{F}_0(a,\lambda)\}_{a\in\{0,1\}^*, \lambda\in\mathbb{N}}\}$ and $\{\mathcal{F}_1(a,\lambda)\}_{a\in\{0,1\}^*, \lambda\in\mathbb{N}}\}$ are said to be computational indistinguishable, if for every non-uniform polynomial-time algorithm $\mathcal{A}$, there exits a negligible function $\mathsf{negl}(\lambda)$, such that for every $a\in\{0,1\}^*$ and every $\lambda\in\mathbb{N}$,
\begin{equation*}
	|\Pr[\mathcal{A}(\mathcal{F}_0(a,\lambda))=1]|-|\Pr[\mathcal{A}(\mathcal{F}_1(a,\lambda))=1]|\leq\mathsf{negl}(\lambda).
\end{equation*}
\end{definition}


\begin{definition}[Simulation-based Security]
Let $\mathcal{F}=(\mathcal{F}_0, \mathcal{F}_1)$ be a functionality, we say a protocol $\pi$ securely computes $\mathcal{F}$ in the presence of static semi-honest adversaries if there exists a probabilistic polynomial-time algorithm $\mathcal{S}_0$ and $\mathcal{S}_1$ such that
\begin{equation*}
    \begin{split}
    \{(\mathcal{S}_0(1^\lambda, x, \mathcal{F}_0(x, y)), \mathcal{F}(x,y))\} \overset{c}\equiv 
    \{(\mathsf{view}^\pi_0(\lambda, x, y), \mathsf{output}^\pi(\lambda, x, y))\},\\
    \{(\mathcal{S}_1(1^\lambda, y, \mathcal{F}_1(x, y)), \mathcal{F}(x,y))\} \overset{c}\equiv 
    \{(\mathsf{view}^\pi_1(\lambda, x, y), \mathsf{output}^\pi(\lambda, x, y))\},
    \end{split}
\end{equation*}
where $x,y$ are inputs from $P_0$ and $P_1$ separately.
\end{definition}



\begin{definition}[IND-CPA Security Game]
A public-key encryption scheme is said to be IND-CPA secure if for all probabilistic polynomial-time adversary $\mathcal{A}$,
\begin{equation*}
    \Pr[\mathsf{Game}^\mathcal{A}(1^\lambda)=1]\leq \frac{1}{2} + \mathsf{negl}(\lambda),
\end{equation*}
where the IND-CPA$^\mathcal{A}(\lambda)$ is defined as follows:
\end{definition}


\protocol{IND-CPA$^\mathcal{A}(\lambda)$}{
b \sample \bin\\
(\pk, \sk)\sample \kgen (1^\lambda)\\
(\state, m_0, m_1) \sample \adv(1^\lambda, \pk, c)\\
c \sample \enc(\pk, m_b)\\
b' \sample \adv(1^\lambda, \pk, c \state)\\
\pcreturn b'=b
}


\subsection{Proofs of Lemma 1 and Lemma 2}
%Next, we prove lemma 1 and lemma 2.

\begin{lemma}
The protocol in Figure 5 (i.e. Dense-Sparse Matrix Multiplication with Insensitive Sparsity) is secure in the MPC-hybrid model.
\end{lemma}

\begin{proof}
We use simulation-based proof \cite{lindell2017simulate} for Lemma 1. Since we are considering our protocol in the MPC-hybrid model, we assume there are two ideal MPC functionalities $\mathcal{F}_\mathsf{mul}$ and $\mathcal{F}_\mathsf{add}$, where $\mathcal{F}_\mathsf{mul}$ takes $[x]_0, [y]_0$ from $P_0$, and $[x]_1, [y]_1$ from $P_1$, and returns $[z]_0$ to $P_0$ and $[z]_1$ to $P_1$ such that $z=xy$,. Similarly, $\mathcal{F}_\mathsf{add}$ takes $[x]_0, [y]_0$ from $P_0$, and $[x]_1, [y]_1$ from $P_1$, and returns $[z]_0$ to $P_0$ and $[z]_1$ to $P_1$ such that $z=x+y$. The security of $\mathcal{F}_\mathsf{mul}$ and $\mathcal{F}_\mathsf{add}$ says that $[z]_0$ and $[z]_1$ are indistinguishable from uniform randomness from the sole view of $P_0$ or $P_1$ separately. That is to say, for all $c\in\mathbb{Z}_\delta$
\begin{equation*}
    \begin{split}
    |\Pr[[\mathcal{F}_\mathsf{mul}([x], [y])]_i=c] - \Pr[r=c]|=0,\\
    |\Pr[[\mathcal{F}_\mathsf{add}([x], [y])]_i=c] - \Pr[r=c]|=0,
    \end{split}
\end{equation*}
where $i\in\{0,1\}$, $\delta$ is the share bit length, and $r$ is a uniform random number sampled from $\mathbb{Z}_\delta$.

Therefore, we need to build a simulator $\mathcal{S}_0$ to simulate the view of $P_0$ in protocol $\pi$. Note in our protocol, all the interactions between $P_0$ and $P_1$ come from $\mathcal{F}_\mathsf{mul}$ and $\mathcal{F}_\mathsf{add}$, then we can use $\mathcal{S}_0$ to generate a uniform random value $r\in\mathbb{Z}_\delta$ for each stage independently. Given that the outputs of ideal functionalities $\mathcal{F}_\mathsf{mul}$ and $\mathcal{F}_\mathsf{add}$ are indistinguishable from uniform randomness for both view of the parties, this simulation works for both $\mathcal{S}_0$ and $\mathcal{S}_1$, and the simulation completes.
\end{proof}



\begin{lemma}
The protocol in Figure 6 (i.e. Dense-Sparse Matrix Multiplication with Sensitive Sparsity) is secure in the PIR-hybrid model with the leakage of $|l_y|$.
\end{lemma}

\begin{proof}
We also use simulation-based proof \cite{lindell2017simulate} for Lemma 2. First, we assume there is a ideal functionality $\mathcal{F}_\mathsf{pir}$, which takes a value set $\mathsf{DB}$ from $P_0$, an index $i$ from $P_1$, and returns $\mathsf{DB}_i$ to $P_1$. The security of $\mathcal{F}_\mathsf{pir}$ are biased since PIR only aim to hide the query $i$ from $P_0$. More formally, the security of single-database computational PIR says that, for every distinct $i,j\in[n]$ and every probabilistic polynomial-time (PPT) adversary $\mathcal{A}$,
\begin{equation*}
        |\Pr[\mathcal{A}(1^\lambda, \mathcal{F}_\mathsf{pir}(i,r))=1]-
        \Pr[\mathcal{A}(1^\lambda, \mathcal{F}_\mathsf{pir}(j,r))=1]|\leq \mathsf{negl}(\lambda),
\end{equation*}
where $\lambda$ is the computational security parameter, $n$ is the size of the database $\mathsf{DB}$, and $\mathsf{negl}$ is a negligible function bounded by computational security parameter $\lambda$.

Since in the offline phase, $P_0$ only sends the public key $pk$ to $P_1$, the simulation for offline phase is trivial. For online phase, we build simulator $\mathcal{S}_0$ and $\mathcal{S}_1$ for $P_0$ and $P_1$ separately.

\textbf{Simulator $\mathcal{S}_0$}: First, for step 1-3, $P_0$ and $P_1$ invokes $\mathcal{F}_\mathsf{pir}$ $|l_y|$ times (which is the pre-defined leakage). $\mathcal{S}_0$ can simulate this process by inputing $\mathcal{F}_\mathsf{pir}$ with $|l_y|$ random encryptions, i.e. $\mathsf{DB}=\{\mathsf{Enc}_{pk}(r_1),...,\mathsf{Enc}_{pk}(r_n)\}$, where $r_1,..,r_n\in\mathbb{Z}_\delta$ are uniform random numbers. For the view of $\mathcal{S}_0$, IND-CPA security says that with a PPT adversary $\mathcal{A}$ who can access the encryption oracle,
\begin{equation*}
    |\Pr[\mathcal{A}(1^\lambda, \mathsf{Enc}_{pk}(\mathsf{DB}_i))=1]-
    \Pr[\mathcal{A}(1^\lambda, \mathsf{Enc}_{pk}(r))=1]|\leq \mathsf{negl}(\lambda).
\end{equation*}
Therefore, from the view of $\mathcal{S}_0$ is indistinguishable from a random encryption with leakage of $|l_y|$. For the rest of the protocol, party $P_0$ sends nothing. The simulation completes.

\textbf{Simulator $\mathcal{S}_1$}: First, for step 1-3, $\mathcal{S}_1$ invokes $\mathcal{F}_\mathsf{pir}$ $|l_y|$ times. Assuming the secure instantiation of $\mathcal{F}_\mathsf{pir}$, the simulation for $\mathcal{S}_1$ in step 1-3 is trivial. Then at step 4, $\mathcal{S}_1$ generates a random value $r\in\mathbb{Z}_\delta$, encrypts it with $P_0$'s public key $\mathsf{Enc}_{pk}(r)$, and sends the result to $P_0$. Observe that for all $c\in\mathbb{Z}_\delta$, for a given $m\in\mathbb{Z}_\delta$,
\begin{equation*}
    |\Pr[r=c] - \Pr[m-r=c]|=0.
\end{equation*}
The simulation completes.
\end{proof}





==> sections/a-3.tex <==
% \section{Generalizing to SVD++}

==> sections/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? 
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} 
    
Our proposed sparse-aware secure cross-domain social recommendation model is customized to a classic factorization based social recommendation models, i.e., Soreg \cite{ma2011recommender}. 
%
We did not choose the state-of-the-art social recommendation model, e.g., deep neural network based model \cite{chen2019efficient}, since it contains complicated non-linear computations and will suffer from serious efficiency problem when involving secure multi-party computation techniques. 

  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}

Our proposed model can be used to build cross-domain social recommendation model while protecting the data privacy of both domains.
%
The proposed sparse-aware matrix multiplication protocols can be widely used to other machine learning scenarios besides social recommendation model. 
%
This paper could shed light on the future research direction of recommendation area. 
%
To our knowledge, our work does not have any potential negative societal impacts.     

  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
We assume that all participants are semi-honest, we also prove the security of our protocols using simulation-based technique.
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
Please find the proof details in the technical appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tikz/pir.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp7209825524397853] 
\draw   (10,16) -- (430,16) -- (430,136) -- (10,136) -- cycle ;
%Straight Lines [id:da7022199441992791] 
\draw    (170,74) -- (238,74) ;
\draw [shift={(240,74)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4987971078393343] 
\draw    (240,110) -- (172,110) ;
\draw [shift={(170,110)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (19,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Client}};
% Text Node
\draw (359,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Server}};
% Text Node
\draw (21,52.4) node [anchor=north west][inner sep=0.75pt]    {\small $q\leftarrow \mathsf{PIR.Query}( i)$};
% Text Node
\draw (230,82.4) node [anchor=north west][inner sep=0.75pt]    {\small $r\leftarrow \mathsf{PIR.Response}(\mathsf{DB} ,q)$};
% Text Node
\draw (21,112.4) node [anchor=north west][inner sep=0.75pt]    {\small $d_i\leftarrow \mathsf{PIR.Extract}( r)$};
% Text Node
\draw (201,52.4) node [anchor=north west][inner sep=0.75pt]    {\small $q$};
% Text Node
\draw (201,117.4) node [anchor=north west][inner sep=0.75pt]    {\small $r$};


\end{tikzpicture}
